Efficient Algorithms for Euclidean Steiner Minimal Tree on Near-Convex Terminal Sets

The Euclidean Steiner Minimal Tree problem takes as input a set $\mathcal P$ of points in the Euclidean plane and finds the minimum length network interconnecting all the points of $\mathcal P$. In this paper, in continuation to the works of Du et al. and Weng et al., we study Euclidean Steiner Minimal Tree when $\mathcal P$ is formed by the vertices of a pair of regular, concentric and parallel $n$-gons. We restrict our attention to the cases where the two polygons are not very close to each other. In such cases, we show that Euclidean Steiner Minimal Tree is polynomial-time solvable, and we describe an explicit structure of a Euclidean Steiner minimal tree for $\mathcal P$. We also consider point sets $\mathcal P$ of size $n$ where the number of input points not on the convex hull of $\mathcal P$ is $f(n) \leq n$. We give an exact algorithm with running time $2^{\mathcal{O}(f(n)\log n)}$ for such input point sets $\mathcal P$. Note that when $f(n) = \mathcal{O}(\frac{n}{\log n})$, our algorithm runs in single-exponential time, and when $f(n) = o(n)$ the running time is $2^{o(n\log n)}$ which is better than the known algorithm stated in Hwang et al. We know that no FPTAS exists for Euclidean Steiner Minimal Tree unless P=NP, as shown by Garey et al. On the other hand FPTASes exist for Euclidean Steiner Minimal Tree on convex point sets, as given by Scott Provan. In this paper, we show that if the number of input points in $\mathcal P$ not belonging to the convex hull of $\mathcal P$ is $\mathcal{O}(\log n)$, then an FPTAS exists for Euclidean Steiner Minimal Tree. In contrast, we show that for any $\epsilon \in (0,1]$, when there are $\Omega(n^{\epsilon})$ points not belonging to the convex hull of the input set, then no FPTAS can exist for Euclidean Steiner Minimal Tree unless P=NP.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}



==> preamble.tex <==
%generic%%%
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{wasysym}
\usepackage{bm}

%%%pagewise footnote numbering%%%
\makeatletter
\@addtoreset{footnote}{section}
\makeatother
%%%%%%%%%%%

\usepackage{tikz}
\usepackage{thm-restate}

\usetikzlibrary{shapes.geometric,matrix,shapes,arrows,positioning,chains}
\usepackage[normalem]{ulem}
\newcommand{\longversion}[1]{#1}
\newcommand{\shortversion}[1]{}
\newcommand{\bigoh}{{\mathcal{O}}}
\usepackage{todonotes}
\usepackage{gensymb}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{xcolor}
\usepackage{boxedminipage}
\usepackage{float}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{stmaryrd,bbm}
\usepackage{environ}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1} \ }}
\newcommand{\mypara}[1]{\smallskip\noindent{\textbf{\sffamily #1} \ }}

%%complexity classes%%%
\newcommand{\NP}{\textsf{NP}}
\newcommand{\NPp}{${\sf NP}$}
\newcommand{\classP}{\textsf{P}}
\newcommand{\APX}{\textsf{APX}}
\newcommand{\FPTAS}{\textsf{FPTAS}}
\newcommand{\FPT}{{\rm \textsf{FPT}}}
\newcommand{\coNP}{\text{\normalfont co-NP}}
\newcommand{\XP}{\text{\normalfont XP}}
\newcommand{\W}[1][xxxx]{\text{\normalfont W[#1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
%%%%

%%problem definition box

\newcommand{\defparproblem}[4]{
  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
  }
  \vspace{1mm}
}

\newcommand{\defproblem}[3]{
  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
  }
  \vspace{1mm}
}

%%

%%useful math macros%
\newcommand{\C}[1]{\mathcal{#1}}
\newcommand{\SC}[1]{\mathscr{#1}}
\newcommand{\BB}[1]{\mathbb{#1}}
\newcommand{\what}{\widehat}
\newcommand{\wtilde}{\widetilde}
%%%%%%%%%%%%%%%%%%%%%

%%%generic fpt paper macros%

%\newtheorem*{theorem*}{Theorem}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{claim}{Claim}[section]
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{observation}{Observation}[section]
%\newtheorem{proposition}{Proposition}[section]
\newcounter{reduction}
\setcounter{reduction}{0}

\newcounter{markingrule}
\setcounter{markingrule}{0}

\newtheorem{mschm}[markingrule]{Marking Scheme}
\newtheorem{redr}[reduction]{Reduction Rule}
\newtheorem{marule}[markingrule]{Marking Rule}

\newcounter{hypothesis}
\setcounter{hypothesis}{0}

\newtheorem{hypo}[hypothesis]{Conjecture}

\newcommand{\Yes}{\textsf{yes}}
\newcommand{\No}{\textsf{no}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Paper specific macros%

\newcommand{\BTJ}{\textsc{Bipartite Token Jumping}}
\newcommand{\Biclique}{\textsc{Bi-clique}}
\newcommand{\MBB}{\textsc{Maximum Balanced Biclique}}
\newcommand{\optbiclq}{{\sf opt}\mbox{-}{\sf biclq}}
\newcommand{\TSAT}{\textsc{$3$-SAT}}
\newcommand{\TD}{\textsc{Skew Detection}} 
\newcommand{\BTS}{\textsc{Bipartite Skew Subgraph}}
\newcommand{\BTIS}{\textsc{Bipartite Skew Induced-Subgraph}}
\newcommand{\BTCS}{\textsc{Bipartite Skew (Induced-)Subgraph}}
\newcommand{\TJ}{\textsc{Token Jumping}} 
%%%%%%%%%%%%%%%%%%%%%%%%


==> preliminaries.tex <==
\section{Preliminaries} \label{preliminaries}

 Consider two regular $n$-gons with vertex sets $\{A_1,A_2,\ldots, A_n\}$ and $\{B_1,B_2,\ldots, B_n\}$, respectively. We denote $A_1A_2A_3...A_n$ and $B_1B_2B_3...B_n$. Without loss of generality, we assume that $\overline{A_iA_{i + 1}} = 1$ for $1 \le i < n$, and $\overline{B_iB_{i + 1}} = \lambda $ for $1 \le i < n$, where $\lambda > 1$. For convenience, we define $A_{n + 1} := A_1$, $B_{n + 1} := B_1$, $A_0 := A_n$ and $B_0 := B_n$. Further, we define $O$ to be the common centre of $A_1A_2A_3 \ldots A_n$ and $B_1B_2B_3 \ldots B_n$. In this paper, we would be using the notation $\{A_i\}$ to denote the polygon $A_1A_2A_3 \ldots A_n$ and $\{B_i\}$ to denote the polygon $B_1B_2B_3 \ldots B_n$. \\

Moreover, we will use the following facts from \cite{hwang1992steiner} extensively.

\begin{lemma} \label{atleast_120}
    (a) No two edges of an SMT can meet at an angle less than $\frac{2 \pi}{3}$. (b) Each Steiner point of an SMT is of degree exactly three.
\end{lemma}

From these two facts, we see that:

\begin{lemma}
    Two edges meeting at a Steiner point must make an angle of $\frac{2 \pi}{3}$.
\end{lemma}

We start by defining some preliminary notations

\begin{definition}
    In our setting, by \textbf{terminal point} or simply \textbf{terminal}, we mean any point in $\{A_i\} \cup \{B_i\}$.
\end{definition}

\begin{definition}
    For any tree $\mathcal T$ on the Euclidean Plane, we denote by the notation $|\mathcal T|$, the sum of lengths of all edges in $\mathcal T$. 
\end{definition}

==> sqaure.tex <==




\section{SMT for two Concentric Squares ($n = 4$)} \label{sqaures}


For two concentric and parallel squares $A_1A_2A_3A_4$ and $B_1B_2B_3B_4$, where $B_1B_2B_3B_4$ encloses $A_1A_2A_3A_4$, the SMT of $\{A_1, A_2, A_3, A_4, B_1, B_2, B_3, B_4\}$ has one of two possible topologies. We will discuss the topologies and the values of $\lambda$ corresponding to an SMT of a particular topology.
\todo{SK: why can there not be any other topology?}
\vspace{0.2cm}
\subsection{Topology - I}
\vspace{0.2cm}

The first topology we discuss is when there is a full Steiner subtree connecting $A_1A_2A_3A_4$ and we have edges connecting $A_i$ and $B_i$ for $1 \le i \le 4$. Let us call this topology for $n = 4$ the \emph{Topology - I} denoted by $T^{(4)}_1$.


\begin{figure}[h!]
\centering
\includegraphics[width=5cm]{4_gon_topo1.png}
\caption{ \emph{Topology - I} for $n = 4$ }
\end{figure}

\subsubsection{Construction}

\begin{itemize}
    \item Construct the SMT of the square $A_1A_2A_3A_4$
    \item Join the points $A_i$ and $B_i$ for $1 \le i \le 4$
\end{itemize}

\subsubsection{Analysis}

We observe that the total length of the Steiner tree formed using this topology is:

$$\color{blue}
|T^{(4)}_1| = (1 + \sqrt{3}) + 4 \cdot \frac{(\lambda - 1)}{\sqrt{2}} = 2 \sqrt{2} \lambda + (1 + \sqrt{3} - 2 \sqrt{2})
$$

\vspace{0.2cm}
\subsection{Topology - II}
\vspace{0.2cm}

The second topology we discuss is when there is a full Steiner subtree connecting $A_1A_4B_4B_1$ as well as another full Steiner subtree connecting $A_2A_3B_3B_2$. These two full Steiner subtrees are in turn connected by a single edge $A_1A_2$, giving us the final Steiner tree. Let us call this topology for $n = 4$ the \emph{Topology - II} denoted by $T^{(4)}_2$.


\begin{figure}[h!]
\centering
\includegraphics[width=5cm]{4_gon_topo2.png}
\caption{ \emph{Topology - II} for $n = 4$ }
\end{figure}

\subsubsection{Construction}

\begin{itemize}
    \item Construct the SMT of the square $A_1A_4B_4B_1$
    \item Construct the SMT of the square $A_2A_3B_3B_2$
    \item Join the points $A_1$ and $A_2$
\end{itemize}

\subsubsection{Analysis}

We observe that the total length of the Steiner tree formed using this topology is:

$$\color{blue}
|T^{(4)}_2| = (1 + \sqrt{3}) \cdot \lambda + 4 \cdot \frac{1}{\sqrt{3}} - \frac{1}{\sqrt{3}} = (1 + \sqrt{3}) \cdot \lambda + \sqrt{3}
$$

\vspace{0.2cm}
\subsection{Topology-I vs Topology-II}
\vspace{0.2cm}

We wish to find the range of $\lambda$ for which Topology-I is better than Topology-II that is $|T^{(4)}_1| < |T^{(4)}_2|$.

\begin{align*}
    & |T^{(4)}_1| < |T^{(4)}_2| \\ 
    \Longleftrightarrow & 2 \sqrt{2} \lambda + (1 + \sqrt{3} - 2 \sqrt{2}) < (1 + \sqrt{3}) \cdot \lambda + \sqrt{3} \\ 
    \Longleftrightarrow & (2 \sqrt{2} - 1 - \sqrt{3}) \cdot \lambda <  (2 \sqrt{2} - 1) \\ 
    \Longleftrightarrow & \lambda <  \frac{(2 \sqrt{2} - 1)}{(2 \sqrt{2} - 1 - \sqrt{3})}
\end{align*}

Therefore, whenever $\lambda <  \Bigg( \dfrac{2 \sqrt{2} - 1}{2 \sqrt{2} - 1 - \sqrt{3}} \Bigg) \approx 18.972$, \emph{Topology-I} produces the SMT; and in other cases \emph{Topology-II} produces the SMT.


